Channel Knowledge Map for Cellular-Connected UAV via Binary Bayesian Filtering

Channel knowledge map (CKM) is a promising technology to enable environment-aware wireless communications and sensing. Link state map (LSM) is one particular type of CKM that aims to learn the location-specific line-of-sight (LoS) link probability between the transmitter and the receiver at all possible locations, which provides the prior information to enhance the communication quality of dynamic networks. This paper investigates the LSM construction for cellularconnected unmanned aerial vehicles (UAVs) by utilizing both the expert empirical mathematical model and the measurement data. Specifically, we first model the LSM as a binary spatial random field and its initial distribution is obtained by the empirical model. Then we propose an effective binary Bayesian filter to sequentially update the LSM by using the channel measurement. To efficiently update the LSM, we establish the spatial correlation models of LoS probability on the location pairs in both the distance and angular domains, which are adopted in the Bayesian filter for updating the probabilities at locations without measurements. Simulation results demonstrate the effectiveness of the proposed algorithm for LSM construction, which significantly outperforms the benchmark scheme, especially when the measurements are sparse.

==> OPD.tex <==
\section{ Data collection optimization for Link State Mapping}\label{sec:LocOpt}

{\color{red} The rest has not been update}

%\begin{figure}[h]%\label{F: PricipleGrid}
%	\centering
%	\includegraphics[scale=0.5]{Pictures/3Dgrid.pdf}
%	\caption{PricipleGrid}
%	\label{F: PricipleGrid}
%\end{figure}

In this section, we intend to optimize data collection location $ \textbf{X}$. 
% Before data collection, the KL-divergence $ KL(\mathcal{T};\mathcal{M}_0) $ between the ground-truth LSM and prior LSM is determined by the
% existing prior LOS distribution \eqref{eq:LoSModel}.
We wish to minimize the  $ KL(\mathcal{T};\mathcal{M}) $ between the ground-truth LSM and the constructed probabilistic LSM in \eqref{eq:OP1} after data collection. 
However, the ground-truth LSM $ \mathcal{T}$ is not available before mapping.
Thus, the mapping performance  can not be evaluated by \eqref{eq:OP1}.
%Naturally, we desire to find a certain optimization metric about $ \mathcal{M} $ and $ \mathcal{M}_0$, and then optimize it so that  $  KL(\mathcal{T};\mathcal{M})$ is as small as possible. 
Hence, we propose to optimize the measurement locations by maximizing  the mutual information between the LSM $ \mathcal{M} $ with the prior LoS probability $ \mathcal{M}_0 $ and the measurement $ \mathbf{Z} $. Then, we propose an efficient algorithm to reduce the computational complexity by transforming the complex high-dimensional computational problem into a sequential search for data collection locations. And finally, we further simplify the problem by setting up a binary detector that converts the complicated integrals that need to be computed into a binary summation, so that we can easily obtain the measured position.
	
At this work, mutual information (MI) of LSM is defined as the expected reduction in entropy regarding all binary LoS random
variable in $ \mathcal{X}_h $ due to observation of another variable, i.e measurements $ \mathbf{Z} $.
\begin{definition} (Mutual information of LoS Map after measuring $ \mathbf{Z} $)
	Let $ I(\mathcal{M},\mathbf{Z}) $ be Mutual information of LSM, which is defined as the intergral of mutual information each location $ \mathbf{x} \in \mathcal{X}_h $ after measuring $ \mathbf{Z} $. %Denote by mutual information of LSM as
	Denote the mutual information of LSM map as follows
	\begin{align}
		I(\mathcal{M},\mathbf{Z})=\int_{\mathbf{x} \in \mathbf{X}_h} I(l(\mathbf{x});\mathbf{Z}) d\mathbf{x}
		\label{eq:definitionMI}
	\end{align}
	where the mutual information evaulate how much the map uncertainty reduces after measuring $ \mathbf{Z}$, $ \mathcal{M}_0 $ is the initial random field of LSM, $ I(l (\mathbf{x}); \mathbf{Z} ) $ is mutual information at location $ \mathbf{x} $ after measuring $ \mathbf{Z} $. 
\end{definition}
We can write the mutual information $ I(l(\mathbf{x}),\mathbf{Z}) $ (See e.g. \cite[p.42]{williams2007information}) as 

\begin{align}
	I(l(\mathbf{x}),\mathbf{Z}) &= H(l(\mathbf{x})) - H(l(\mathbf{x})| \mathbf{Z})  \label{eq:definitionMILoc}\\
	&= H(l(\mathbf{x})) - \int_{\mathbf{Z} } p(\mathbf{Z} = \textbf{o}_N)H(l(\mathbf{x}) | \mathbf{Z} = \textbf{o}_N) d\mathbf{Z}\nonumber
\end{align}

where $ H(l(\mathbf{x})) = -\sum_c \Pr(l(\mathbf{x})=c)\ln(\Pr(l(\mathbf{x})=c))$ is the entropy of prior LSM, and its prior probability $ \mathcal{M}_0 $ or $ \Pr(l(\mathbf{x})=c) $ can be calculated by \eqref{eq:LoSModel},

\begin{definition} (Conditional mutual information of LSM measuring $ z_n $ under the known $ \mathbf{Z}_{n-1}=\mathbf{o}_{n-1} $)
	
	Let  $ I(\mathcal{M};z_n|\mathbf{Z}_{n-1}=\mathbf{o}_{n-1}) $ and $ I(l(\mathbf{x});z_n|\mathbf{Z}_{n-1}=\mathbf{o}_{n-1}) $  be conditional mutual information of LSM and condition mutual information LoS bianray random variable at location $ \mathbf{x} $ ,respectively, i.e., in the case of conditioning on a particular value $ \mathbf{Z}_{n-1}=\mathbf{o}_{n-1} $,
 	 \begin{align}\label{eq:definitionCMILSM}
 	 	%&I(\mathcal{M};z_n|\mathbf{Z}_{n-1}=\mathbf{o}_{n-1}) \nonumber \\
 	 %	=&\int_{\mathbf{x} \in \mathbf{X}_h} I(l(\mathbf{x});z_n|\mathbf{Z}_{n-1}=\mathbf{o}_{n-1}) d\mathbf{x}
 	 		&I(\mathcal{M};z_n|\mathbf{Z}_{n-1}=\mathbf{o}_{n-1}) \nonumber\\
 	 		=&\int_{\mathbf{x} \in \mathbf{X}_h} I(l(\mathbf{x});z_n|\mathbf{Z}_{n-1}=\mathbf{o}_{n-1}) d\mathbf{x}  \\
 	 		&I(l(\mathbf{x});z_n|\mathbf{Z}_{n-1}=\mathbf{o}_{n-1})\nonumber \\
 	 		=&H(l(\mathbf{x})|\mathbf{Z}_{n-1}=\mathbf{o}_{n-1})-H(l(\mathbf{x}|z_n,\mathbf{Z}_{n-1}=\mathbf{o}_{n-1}))\nonumber
 	 \end{align}
	where conditional entropy $ H(l(\mathbf{x})|\mathbf{Z}_{n-1}=\mathbf{o}_{n-1}) $ and $ H(l(\mathbf{x})|z_n,\mathbf{Z}_{n-1}=\mathbf{o}_{n-1})) $ can be given by, 
		\begin{align}\label{eq:definitionCMILoc}
			&H(l(\mathbf{x})|\mathbf{Z}_{n-1}=\mathbf{o}_{n-1}) \nonumber\\
			=& -\sum_c \Pr(l(\mathbf{x})=c|\mathbf{Z}_{n-1}=\mathbf{o}_{n-1})\ln \Pr(l(\mathbf{x})=c|\mathbf{Z}_{n-1}=\mathbf{o}_{n-1}) \nonumber\\
			&H(l(\mathbf{x})|z_n,\mathbf{Z}_{n-1}=\mathbf{o}_{n-1})) \\
			=&\int \sum_c \Pr(z_n|\mathbf{Z}_{n-1}) \Pr(l(\mathbf{x})=c|z_n,\mathbf{Z}_{n-1}=\mathbf{o}_{n-1}) \nonumber\\
			& \ln \Pr(l(\mathbf{x})=c|z_n,\mathbf{Z}_{n-1}=\mathbf{o}_{n-1})  d z_n \nonumber
		\end{align}   

  	 
\end{definition}

%\subsection{Basic definition}
%\begin{definition} (What is LSM after measuring $ \mathbf{Z}_n $)
%	We denote $ \mathcal{M}_n $ by the probability distribution of random field after measuring $ Z_{n} $
%	We denote $ \mathcal{M}_n $ by the random field at $ n $-th interval, whose probability distribution would be given by the algorithm of Section~\ref{sec:Mapping} and the prior LoS distribution \eqref{eq:LoSModel}.
%\end{definition}


\subsection{Problem Formulation}
For this challenge, our main idea is to reduce the uncertainty of probabilistic LSM $ \mathcal{M} $. 
In previous mapping and sensor studies \cite{romero2020aerial,williams2007information}, the maximum
mutual information criterion(MMI) has been studied a lot.
 Similar to the MMI criterion, the following
optimization problem about maximizing the uncertainty reduction of probabilistic LSM $ \mathcal{M} $ with the measurement $ \mathbf{Z}$ is established to find $ N$ measurements location $ \textbf{X}$
%so that  optimize the mapping performance.
\begin{equation}\label{eq:OP2}
	\begin{aligned}
		\textbf{(P2)}:	\mathop{max}\limits_{\mathbf{X} } 	\quad I(\mathcal{M};\mathbf{Z})
	\end{aligned}
\end{equation}
In order to solve the above problem, it is necessary to calculate the posterior probability $ \Pr(l(\mathbf{x})|\mathbf{Z}=\mathbf{o}_N)$ and $ \Pr(\mathbf{Z}=\mathbf{o}_N) = \prod_{\mathbf{x}_n \in \mathbf{X}} \sum_c p_{z|c}(\mathbf{x}_n)\Pr(l(\mathbf{x}_n)=c)  $, for any $ \mathbf{o}_N \in \mathbb{R}^N, c \in \{0,1\} $ according to \eqref{eq:definitionMI} and \eqref{eq:definitionMILoc}.
Therefore, the calculation of $ I(\mathcal{M};\mathbf{Z}) $ would include the multi-dimensional integral and complex combinatorial problem, which has high computatinal complexity when the measurement number  $ N $ is large.

%{\color{red}
%Another optimization metric is 	directly to maximize the KL-divergence $ KL(\mathcal{M};\mathcal{M}_0)$ between $ \mathcal{M}$ and $ \mathcal{M}_0$
%, 
%\begin{equation}\label{eq:OP3}
%	\begin{aligned}
%		\textbf{(P3)}:	\mathop{max}\limits_{\textbf{X} } \quad  KL(\mathcal{M};\mathcal{M}_0)
%	\end{aligned}
%\end{equation}
%even if the equation $KL(\mathcal{T}(\mathbf{x})||\mathcal{M}_0(\mathbf{x})) = KL(\mathcal{T}(\mathbf{x})|| \mathcal{M}(\mathbf{x})) +
%KL(\mathcal{M}(\mathbf{x})||\mathcal{M}_0(\mathbf{x})) $ will not be satisfied in general. The KL-divergence $ KL(\mathcal{M};\mathcal{M}_0) $ can be evaluated by 
%\begin{equation}\label{eq:KL_M0_M}
%	\begin{aligned}
%			KL(\mathcal{M};\mathcal{M}_0) &=\int_{\mathbf{x} \in \mathcal{X}_h}KL(\mathcal{M}(\mathbf{x})||\mathcal{M}_0(\mathbf{x}))d\mathbf{x}\nonumber\\
%			&=\int_{\mathbf{x} \in \mathcal{X}_h} KL(p(l(\mathbf{x})|\mathbf{Z})||p(l (\mathbf{x})))d\mathbf{x}  \\
%			&=\int_{\mathbf{x} \in \mathcal{X}_h} \sum_{c} p(l(\mathbf{x})=c|\mathbf{Z}) \ln \frac{p(l(\mathbf{x})=c|\mathbf{Z})}{p(l(\mathbf{x})=c)} d\mathbf{x}
%			%\\
%		%	&=\int_{\mathbf{x} \in \mathcal{X}_h} I(l (\mathbf{x}); \mathbf{Z} )d\mathbf{x} \\
%	\end{aligned}
%\end{equation}
%
%Since
% $ I(\mathcal{M};Z) := \int_{\textbf{x} \in \mathcal{X}_h} I(l(\textbf{x});\textbf{Z}) d \textbf{x}= \int_{\textbf{x} \in \mathcal{X}_h} \int_{\mathbf{Z}}p(\mathbf{Z})
%KL(p(l (\mathbf{x})  |\mathbf{Z})  \| p(l(\mathbf{x}))) d\mathbf{Z} d \textbf{x}= \int_{\textbf{x} \in \mathcal{X}_h} \int_{\mathbf{Z}}p(\mathbf{Z})KL(\mathcal{M}(\mathbf{x})||\mathcal{M}_0(\mathbf{x}))
% d\mathbf{Z} d \textbf{x}$, 
%$ KL(\mathcal{M};\mathcal{M}_0)$\eqref{eq:OP3} would be better than \eqref{eq:OP2} $ I(\mathcal{M};\mathbf{Z})$ if it can find the maximum value of $ KL(\mathcal{M};\mathcal{M}_0)$, because it has less computation cost.
% %, because it does not require the distribution of $ \mathbf{Z} $. Thus, there is no requirement for whether the channel parameters are known.
% In the previous simulations, we determined that using \eqref{eq:OP2} would improve the quality of the map, but we had not done it with \eqref{eq:OP3}.
%}  
%矢量场的散度在体积τ上的体积分等于矢量场在限定该体积的闭合曲面s上的面积分
%LOS/NLOS binary
%random variable $ l(\textbf{x})$. 
% If we reduce the uncertainty and use the
%correlation between the LOS maps lx , for different x, to reduce
%the error , then the KL-divergence in equation (7) will also
%reduce. 

%
%
%Firstly, we remember to maximize the KL-divergence $ KL(\mathcal{M};\mathcal{M}_0) $, even if the equation $KL(\mathcal{T}(\mathbf{x})||\mathcal{M}_0(\mathbf{x})) = KL(\mathcal{T}(\mathbf{x})|| \mathcal{M}(\mathbf{x})) +
%KL(\mathcal{M}(\mathbf{x})||\mathcal{M}_0(\mathbf{x})) $ will not be satisfied in general. The KL-divergence $ KL(\mathcal{M};\mathcal{M}_0) $ can be evaluated as 
%\begin{equation}\label{eq:KL_M0_M}
%	\begin{aligned}
%		KL(\mathcal{M};\mathcal{M}_0) &=\int_{\mathbf{x} \in \mathcal{X}_h}KL(\mathcal{M}(\mathbf{x})||\mathcal{M}_0(\mathbf{x}))d\mathbf{x}\nonumber\\
%		&=\int_{\mathbf{x} \in \mathcal{X}_h} KL(p(l(\mathbf{x})|\mathbf{Z})||p(l (\mathbf{x})))d\mathbf{x} %\\
%	%	&=\int_{\mathbf{x} \in \mathcal{X}_h} I(l (\mathbf{x}); \mathbf{Z} )d\mathbf{x} \\
%	\end{aligned}
%\end{equation}
%where the fourth "=" is due to the relationship between KL-divergence and mutual information \cite{gfh }.


 %In fact,
%KL-divergence $ KL(\mathcal{M}_0(\mathbf{x})||\mathcal{M}(\mathbf{x})) := KL(p(l(\textbf{x})) \|p(l(\textbf{x})|\mathbf{Z} )) $ is equal to mutual information $I(l(\textbf{x}); \mathbf{Z}) $. %In Numerical results section, we will give the difference between $KL(rx||p(lx)) - KL(rx||p(lx|zxN ))$ and the
%mutual information $ I(lx; zxN ) $ .

% The LOS map construction problem can be written as the following optimization problem
% We want to update the a priori LOS map so that it is as close to the LOSmap as possible
% We have the LOS map 


%For simplicity, denote $ \phi(\textbf{x}_N) =  \int_{0}^{D} I(l_x; \textbf{z}_{\textbf{x}_N}) dx $.
%\eqref{eq:OP2} is a 

%\subsection{Sequentially to search the sub-optimal location}
To settle the calculation problem and sequentially search the data collection location, we consider iteratively to search the measurement location. At $ n-1 $ interval, the distribution of LSM can be evaluated by $ p(l(\mathbf{x})|\mathbf{Z}_{n-1} = \mathbf{o}_{n-1})$, denoted by $ \mathcal{M}_{n-1} $.
Thus, the iteratively maximize conditional mutual information problem can be written as
\begin{equation}\label{eq:OP3}
	\begin{aligned}
		\textbf{(P3)}:	\mathop{max}\limits_{\textbf{x}_n } \quad 
		I(\mathcal{M};z_n|\mathbf{Z}_{n-1}=\mathbf{o}_{n-1})
		 %\int_{\textbf{x} \in \mathcal{X}_h} I(l(\textbf{x});\textbf{z}(\mathbf{x}_n)|\textbf{Z}_{n-1}\}) d \textbf{x}
	\end{aligned}
\end{equation}
However, the probability distribution of $ z_n$ at the location $ \mathbf{x}_n$ depends on the channel model, which is difficult to obtain and unprecise in most cases. In addition, the integral has high computation cost, which still has high demand to the UAV when online mapping is required. Hence, as shown in Fig.\ref{F:Meas2detector}, we introduce the LOS/NLOS indicator output $ m_n $ to alleviate this problem, i.e. $ m_n = \mathcal{H}(z_n,\mathbf{x}_n) $, where $ \mathcal{H}(.) $ is the LOS/NLOS detector by the radio measurements. The sample space of $ m_n $ is $ \{0,1\} $. Denote $ \mathbf{M} = \{m_1,...,m_N\} $ the LOS/NLOS indicator set. 
It can be realized by the binary Gaussian detector \cite{kay1993fundamentals}, as follows  
\begin{figure}[t]
	\centering
	\includegraphics[scale=0.93]{Pictures/Meas2detector.pdf}
	\caption{The link state mapping by the LOS/NLOS detector }
	\label{F:Meas2detector}
\end{figure}

\begin{equation}\label{eq:LOS/NLOSdetector}
	\begin{aligned}
		p(m_n = 1 | l(\mathbf{x}_n) = 1) &=  p(z_n > t(\mathbf{x}_n) | l(\mathbf{x}_n) = 1) \\
		&= 1 - \epsilon_{1,0}(\mathbf{x}_n) \\
		p(m_n = 0 | l(\mathbf{x}_n) = 0) &=  p(z_n \leq t(\mathbf{x}_n)| l(\mathbf{x}_n) = 0) \\
		&= 1 - \epsilon_{0,1}(\mathbf{x}_n)
	\end{aligned}
\end{equation}
where $ t(\mathbf{x}_n) $ is the detector threshold setting that determine the miss alarm rate and false alarm rate,
\begin{equation}\label{eq:faslealarmandmissalarm}
	\begin{aligned}
		&\epsilon_{1,0}(\mathbf{x}_n) 
	%	= \int_{-\infty}^{t(\mathbf{x}_n)}& \frac{1}{\sqrt{2\pi (\sigma_{1}^2+\sigma^2)}}e^{-\frac{(z(\mathbf{x}_n) - \mu_1(\mathbf{x}_n))^2}{2(\sigma_{1}^2+\sigma^2)}} dz(\mathbf{x}_n) \\
		= 1 - Q(\frac{z(\mathbf{x}_n) -\mu_1(\mathbf{x}_n) }{\sqrt{\sigma_{1}^2+\sigma^2}}) \\
		& \epsilon_{0,1}(\mathbf{x}_n) 
	%	&= \int_{t(\mathbf{x}_n)}^{\infty}& \frac{1}{\sqrt{2\pi (\sigma_{0}^2+\sigma^2)}}e^{-\frac{(z(\mathbf{x}_n) - \mu_0(\mathbf{x}_n))^2}{2(\sigma_{0}^2+\sigma^2)}} dz(\mathbf{x}_n) 
	=  Q(\frac{z(\mathbf{x}_n) -\mu_0(\mathbf{x}_n) }{\sqrt{\sigma_{0}^2+\sigma^2}})
	\end{aligned}
\end{equation}
For simplicity, we set the detector threshold to be half the sum of $ \mu_1(\mathbf{x}_n) $ and $ \mu_0(\mathbf{x}_n) $, i.e. $ t(\mathbf{x}_n) = \frac{\mu_1(\mathbf{x}_n) + \mu_0(\mathbf{x}_n)}{2} $.
Thus, the optimization problem in \eqref{eq:OP3} can be redefined as 
\begin{equation}\label{eq:OP4}
		\begin{aligned}
		\textbf{(P4)}:	\mathop{max}\limits_{\textbf{x}_n } \quad 
		I(\mathcal{M};m_n|\mathbf{M}_{n-1}=\mathbf{q}_{n-1})
		 %\int_{\textbf{x} \in \mathcal{X}_h} I(l(\textbf{x});m(\mathbf{x}_n)|\textbf{m}_{n-1}\}) d \textbf{x}
	\end{aligned}
\end{equation}
where $ \mathbf{q}_{n-1} $ is a real sample of random vector $ \mathbf{M}_{n-1} $ at the last $ n-1 $ intervals, $ \mathbf{q}_{n-1} \in  \{0,1\}^{n-1} $ . The calculation of $ I(\mathcal{M};m_n|\mathbf{M}_{n-1}=\mathbf{q}_{n-1}) $ requires reference to \eqref{eq:definitionCMILSM} - \eqref{eq:definitionCMILoc}, which requires the substitution of probabilities $ \Pr(l(\mathbf{x})=c|m_n,\mathbf{M}_{n-1}=\mathbf{q}_{n-1})$, $ \Pr(l(\mathbf{x})=c|\mathbf{M}_{n-1}=\mathbf{q}_{n-1})$ and $ \Pr(m_n|\mathbf{M}_{n-1}) $  for  $ \Pr(l(\mathbf{x})=c|z_n,\mathbf{Z}_{n-1}=\mathbf{o}_{n-1})$, $ \Pr(l(\mathbf{x})=c|\mathbf{Z}_{n-1}=\mathbf{o}_{n-1})$ and $ \Pr(z_n|\mathbf{Z}_{n-1}) $, respectively, in the equations. 
The calculation of $ \Pr(l(\mathbf{x})=c|\mathbf{M}_{n-1}=\mathbf{q}_{n-1})$, $ \Pr(m_n|\mathbf{M}_{n-1}) $ and $ \Pr(l(\mathbf{x})=c|m_n,\mathbf{M}_{n-1}=\mathbf{q}_{n-1})$ refers to Appendix \ref{Appendix C}.

Taking 1D LSM mapping as an example, the conditional mutual information $ I(\mathcal{M};m_1) $ with respect to $ \|\mathbf{x}_1 \|$ is shown in the Fig.\ref{F: MI_initial}, where the prior LoS probability is given by \eqref{eq:LoSModel}. From the above figure, it can be seen that there is a maximum value $ \hat{\mathbf{x}}_1$ of $ I(\mathcal{M};m_1)$.

\begin{figure}[h]
	\centering
	\includegraphics[scale=0.7]{Pictures/MI_initial.pdf}
	\caption{The Mutual information $ I(\mathcal{M};m_1)$ in different measurement location, $ \|\mathbf{x}_1 \| \in [0,1000]$.}
	\label{F: MI_initial}
\end{figure}

\subsection{Iteratively search for the sub-optimal measurement location via Bisearch}
%Iteratively search for the optimal measurement point via Bisearch

%Since the 

 Since the conditional independence of $ l(\mathbf{x})$ in different angles, the maximum mutual information problem with respect to all the area $ \mathcal{X}_h$ in \eqref{eq:OP4} can be simplified to finding a certain location so that the mutual information in the direction where it is located is maximized, i.e 
 \begin{equation}\label{eq:OP5}
 	\begin{aligned}
 		\textbf{(P5)}:	\mathop{max}\limits_{\textbf{x}_n } \quad 
 		\int_{x \in \mathcal{D}_{\mathbf{x}_n}} I(l(\mathbf{x});m_n|\mathbf{M}_{n-1} = \mathbf{q}_{n-1}) d\textbf{x}
 		%\int_{\textbf{x} \in \mathcal{X}_h} I(l(\textbf{x});m(\mathbf{x}_n)|\textbf{m}_{n-1}\}) d \textbf{x}
 	\end{aligned}
 \end{equation}
 where $ \mathcal{D}_{\mathbf{x}_n} $ represents the set of positions on the ray where the projection of base station and $ \mathbf{x}_n $ are connected towards $ \mathbf{x}_n $. %$ 	
%	I(\mathcal{M}_{n-1};m(\mathbf{x}_n)) = \int_{x \in \mathcal{D}_n} I(\mathcal{M}_{n-1}(\mathbf{x});m(\mathbf{x}_n)) d\textbf{x} $, where $ \mathcal{D}_n$ is the set of locations in the direction of position $ \textbf{x}_n$. 	
For simplicity,	we uniformly divide the GBS outward into  $ M $ direction with an angular interval of $ \delta_{\theta} $, $ M \leq N$. Denote $ \Phi = \{1,2,3,...,M\} $ by the index set of direction. Denote $ \theta_j = (j-1)\delta_{\theta}, j \in \Phi $ by the angle of the direction $ j $. We hope that we can iteratively find the optimal measurement location for probabilistic LSM construction. 
For every $ \theta_j $, we search for an optimal location $ \textbf{p}_{j}$ in this direction, and then find the direction $ i_{n} $ with the largest mutual information $ I_{i_n}:= \int_{x \in \mathcal{D}_{i_n}} I(l(\mathbf{x});m_n|\mathbf{M}_{n-1} = \mathbf{q}_{n-1}) d\textbf{x} $ from $ M $ directions, where $ I_{i_n} \geq I_{j} $, for any $ j \in \Phi$, $ \mathcal{D}_j $ is the set of locations on direction $ j$ . The optimal position $ \textbf{p}_{i_{n}} $ in the optimal direction $ i_n $ is the position we are iteratively looking for at $n$ -th interval . %The maximize mutual information problem with respect to the whole map in \eqref{eq:OP5} can be simplified as find an location in $ M $ direction so that the mutual information with respect to the map in this direction } 
%{\color{blue}Since the conditional independence of $ l(\mathbf{x})$ in different angles, we just consider to maximize the spatial integral $ \int_{\|\textbf{x}\| \in [0,\mathcal{D}_j]} I(\mathcal{M}_{n-1}(\textbf{x});m(\textbf{x}_n)) d\textbf{x}   $ of mutual information $ I(\mathcal{M}_{n-1}(\textbf{x});m(\textbf{x}_n))$ with the location $ x $ which has the same angle $ \theta_j$ to the projection of GBS .}
 %Thus, our probabilistic LSM can be viewed as the sum of multi-1D LSM, we can use the bi-search to find the maximum value of $ \eqref{eq:OP5}$. %Denote $ \mathcal{X}_{h}^b$ the boundary of $ \mathcal{X}_h$, $ \mathcal{X}_{h}^b \subset \mathcal{X}_h$. 
 The iteratively search process for the optimal location selection can be summarized as Algorithm \ref{alg3}



% ,The $ \int_{\|\mathbf{x} \| \in [0,D]} I(\mathcal{M}_{0}(\mathbf{x});m(\mathbf{x}_1))d\textbf{x}$ with respect to $ x_1$ is shown as the Fig. \ref{F: MI_initial}, where the prior probabilites $ P_{j1}(.)$ is given by \cite{priorLSM}.


%=============================Algorithm==========================
\begin{algorithm}
	\caption{Iteratively search for the optimal measurement point for link state mapping via Bisearch}
	\label{alg3}
	\begin{algorithmic}[1]
		\STATE{\textbf{Input:} Prior probability $ \mathcal{M}_{0} $ , The projection  of GBS $ \textbf{x}_{bs} $, The discrete direction number $ M $}
		\STATE{Compute the maximum distance set $ \mathcal{B}:=\{B_j\}_{j=1}^M$,
		$ B_j $ is the distance	to $ \mathbf{x}_{bs}$ direction $ j $.}
		\STATE{Based on \eqref{eq:OP5}, compute the first selected location set $ \mathcal{P}:=\{ \mathbf{p}_{j}\}_{j=1}^M $ in each direction and its corresponding maximize mutual information set $ \mathcal{I}:= \{I_{j}\}_{j=1}^M $ via Bi-search in each direction }.
		\STATE{\textbf{For} $ n=1:N $}
		\STATE{The optimal direction index at $ n $-th intervals $ i_n = \text{argmax}_{j} \ I_{j}$}
		\STATE{The optimal location $ \hat{\textbf{x}}_n  := \textbf{p}_{i_n}$}
		\STATE{Updating the LoS log likelihood ratio $ \mathcal{L}_N(\mathbf{x}) $ at direction $ i_n$ by  binary bayesian filter \eqref{eq:recursiveLn} after measuring the RSS $ z(\mathbf{p}_{i_n}) $ at position $ \textbf{p}_{i_n} $}
		\STATE{Based on \eqref{eq:OP5}, Bi-search for the next optimal location $ \mathbf{p}'_{i_n} $ at direction $ i_n $ and its corresponding maximize mutual information $ I'_{i_n} $ }
		\STATE{$ \mathbf{p}_{i_n} := \mathbf{p}'_{i_n} $, $ I_{i_n} := I'_{i_n} $}
		
		
		\STATE{\textbf{end}}
	\STATE{For the location $ \mathbf{x}$ without updating }
	\STATE{Update the probabilistic LSM $ \mathcal{L}_N(x)$ using spatial interpolation, such as IDW-KNN computed by \eqref{eq:KNNinterpolation}}
	

	\STATE{Compute $ \mathcal{M}(\mathbf{x}) = 1/(1+e^{-\mathcal{L}_N(\mathbf{x})}) $}
		
		
	
	\STATE{\textbf{Output:}} The selected measurement point $ \{\hat{\mathbf{x}}_n\}_{n=1}^{N}$ and constructed LSM  $\mathcal{M}$
	,
	%	\FOR{grid $ l_i$}
	%\STATE{ $lsmlog_{t,i} = lsmlog_{t-1,i} + Inv\_RSS\_sensor\_model(l_i,z_t,\textbf{x}_t)
		%	-l_0 $}
	%	\STATE{xxx}$$x_n
	%	\E$$x_n
\end{algorithmic}
\end{algorithm}
%==================================================================







